A theory of neural emulators

A central goal in neuroscience is to provide explanations for how animal nervous systems can generate actions and cognitive states such as consciousness while artificial intelligence (AI) and machine learning (ML) seek to provide models that are increasingly better at prediction. Despite many decades of research we have made limited progress on providing neuroscience explanations yet there is an increased use of AI and ML methods in neuroscience for prediction of behavior and even cognitive states. Here we propose emulator theory (ET) and neural emulators as circuit- and scale-independent predictive models of biological brain activity and emulator theory (ET) as an alternative research paradigm in neuroscience. ET proposes that predictive models trained solely on neural dynamics and behaviors can generate functionally indistinguishable systems from their sources. That is, compared to the biological organisms which they model, emulators may achieve indistinguishable behavior and cognitive states - including consciousness - without any mechanistic explanations. We posit ET via several conjectures, discuss the nature of endogenous and exogenous activation of neural circuits, and discuss neural causality of phenomenal states. ET provides the conceptual and empirical framework for prediction-based models of neural dynamics and behavior without explicit representations of idiosyncratically evolved nervous systems.

==> sections/adding_empirical_neuroscienes.tex <==


\subsection{ET requires whole-organism neuroscience terminology}
%\subsection{Practical tests for ET}
[STAY Focused: state how ET proposes to operationalize; and what experimental hypothesis it makes]

As an implicit contribution to experimental neuroscience and psychology - ET requires more objective and quantitative descriptions of neural and phenomenal states. In particular, ET proposes that beyond a certain level of \textit{accuracy}, software or hardware \textit{implementations} of models of neural activity must reproduce all \textit{capacities} of biological organisms. We provide working definitions of these terms and below we suggest conceptual frameworks for how these terms can be conceptualized (see Sections 3 and 4):

\begin{itemize}
    \item \textit{Accuracy}: the similarity between states generated by a biological organism and states generated by an emulator or simulator of the organism. Thus, evaluating similarity between phenomenological states requires third-person measurable outputs such as subjective report [cite; Good to link to access vs. phenomenal consciousness; try not to solve everything here...]

    \item \textit{Holistic output}. With respect to accuracy, we add that that evaluating the fit to data needs to be understood in terms that go beyond statistical frameworks already implemented in systems neuroscience and focus on whole-organism neuroscience. In particular, we view that the notion of error [cite] of a model that carries out classification and/or time-series model  is inadequate in framing questions around wholistic emulation or simulation of an organisms. [IT WOULD BE GREAT to link this part to standard models/theoretical neuroscience which do indeed provide statistical descriptions of brain function.]    
    
    \item \textit{Capacity}: the repertoire of outputs that a biological organism is capable of generating that are of some interest for an observer. That is, we reserve "capacity" to refer to whole-organism level behaviors or decision making capabilities and explicitly exclude physical dynamics (e.g. ions moving across neuronal membranes).[YES, this is very important that ET actually focuses on whole organism emulation - not specifically on subsystems and nuances]
    
    \item \textit{Emulator/simulator implementation}: generally any implementation of a model that captures various levels of a biophysical neural system's operations. For clarity, there is no such thing as a "software"-only implementation of a model as all functioning models require physical implementations on computer hardware sources.

\end{itemize}


==> sections/agency.tex <==



- try to start with a central question: what are we trying to copy ? what kinds of systems?
- self-organizing-systems that amount to what we call "lving" organimss, as opposed to any physical system, e.g. cell or atom, or weather patterns which seek equilibria.

- from this perspective, what defines an alive SOS- is the same as what makes most SOSs - namely a locus of causliaty 

- try to think a bit about multicellular organisms and what their goals are... seems keeping cells alive is a central goal... in fact, agency tells us what they all a for biophysical etc agency
all of which are guarantors of or organism survival and gene copying



- basically says consciousness isn't causal - it may just be a phenomenon that occurs given some ... THIS IS A STRONG CLAIM (much written on epiphenomenalism)>
- state the weakest version of this, and perhaps at the end of this section

- does locus of causality here help us?  

= so how do a and b know they are part of the se system?!

maybe locus of causality then can't occur at such small levels... and we need to keep moving up

... so a central proposal is that agency experience is central to being or consciousness and that it can only be computed at some scale or specific query or configuration 

- so we need a definition of sufficiently structured self organizing system that can represent itself and the causal link
- an extreme hypothesis is to say that "we do not care about preserving systems that do not have agency". E.g. perhaps rocks or simple machines, but not completely clear. 

at some level this says that the boundaries of a self organizing system extend to all downstream states that can be "reliably" Co activated?!  ... 

for wbe it essentially means that all states that are cross linked are part of the system?!?!

It has the weird implication that more weird implications that things we learn to do reliably become part of us... agency is thus about bringing many things under control of other things. It seems to suggest that extra-personal things like cultural practices and ... are a type of consciousness ?!!? not super clear...


%\label{submission}
%\input{sections/introduction.tex}

\subsection{Conceptual background: from math to the physics of prediction}

- the best psychological explanation of a life on earth is that they are "self-organizing-systems". biophysical organisms are essentially self-organizing systems. Explain what this means cite correct papers

- the capacity to self organize conceptually requires 2 components: one to understand the locus of causality - what is part of me and what is part of the outside; and 2 - a sufficiently "efficient" capacity for survival valuable/optimized/optimal action selection
- maybe bring in a bit of Max Tegmark's work here to propose that a central principle of life and complex system organization (-> high entropy) is a type of "prediction" processing. 

\textbf{AI systems as prediction machines}. AI safety issue and rethinking them as a specific type of tool...
- another explanatory function is to help us understand what the goals of increasingly powerful prediction systems. 

thought experiment
- there is a strong relations betwee next token prediction in LLMs and WBE. In essence, LLMs predict the next likely token - while WBE's predict the next likely state of the brain and possible behavior state. Critically, LLMs are trained on human behavior - i.e. written text - and the (open secret) is that because flexibility of human language (CITE STUFF) there is simply no next perfect word/token.  In fact, there's no next best perfect sentence - or paragraph.  This isn't how human behavior (or language/verbalization/thought) likely work.

In contrast, WBEs also will have similar behavior with no perfect next state. (Note: chaotic dynamics in healthy brains so this wouldn't work anyways).  That is, we can't really expect exact next state of the world, but this type of thinking is critical.

\subsection{Agency experience and schizophrenia: why synapses do/don't matter}
- we have generally not made much progress in cognitive neuroscience by looking at synapses
- most of what we know comes from... explain
- so why would we think synaptic-activity level copying is required to formulate human experience? !

- indeed, we know a very interesting story of schiziphreani - where wide-brain distributed networks - pathologies are likely driving the agency loss symptoms
- the best 

\subsection{Machine agency and vicarious agency}
- somewhere in this paper need to discuss this sense of agency over other's behaviors
- but also simple stuff like agency over the computer mouse and the keyboard...


==> sections/implications.tex <==
%Our work suggests a number of novel results.  Most prominently, ET proposes that computational systems that implement neural-dynamics based predictive models of sufficient accuracy - will experience conscious states. We provided several empirical arguments for why this occurs. From a theory perspective, we propose that modeling physical causality - may be sufficient for artificial systems to generate internal phenomenal states. ET also proposes that architecture and causality may not be required to accurately model nervous systems. That is, ET proposes that because causality can be simulated using models and that evolution created idiosyncrasies at both the biophysical or anatomical modularity levels may not be necessary requirements for organisms.

%Based on these working definitions we provide the following hypotheses that propose how modeling of biophysical systems can be achieved from empirical data:

%\begin{enumerate}[label={H\arabic*:}, start=1]

    %\item In the "large" data limit, \textit{emulators} will generate all capacities of the source systems including the generation of consciousness.
    
%    \item In the finite-data limit, \textit{emulators} can generate all capacities of the systems they model.
    
 %   \item In the large- or infinite-data limit, \textit{simulators} will generate all capacities of the systems they model.\footnote{We note  that although ET claims that simulators can essentially have "conscious" states, there is a significant burden on such software (only) systems to simulate all (or nearly all) of the capacities of the systems they are simulating. That is, there is implicit assumption in C2 that in order to achieve their behavioral abilities as well as consciousness, biological organisms require a lot of modularization and specialization - and that such requirements will impose constraints on software systems that simulate them. }

%\end{enumerate}

%ET also proposes that emulators are 

%We return to the function $Q$ which describes the time evolution of neural states $x_{i,t}$ under endogenous (i.e. internal state) and exogenous (i.e. external stimuli or inputs) drives. While in  neuroscience we seek mechanistic descriptions for how the system studied evolved from $t-1$ to $t$, we propose that $Q$ can be learned from empirical data without a specific theory:

%\begin{equation}
%    Q = P(x_{i,t} \mid x_{i,t-1}, s_{t-1})
%\end{equation}

%where $i$ stands for a neuronal state.  Most importantly, we propose that in this framework, the $i$s are spatial scale agnostic and can represent individual synapses, neurons but also meso-scale activity (e.g. local-field-potential) or macro-scale activity (e.g. entire anatomical areas such as visual or motor systems). Thus, we envision that the spatial resolution can be set arbitrarily or based on principles discuss most often in Magnetic Resonance Imaging (MRI) brain parcellation methods \cite{eickhoff2018imaging}.

%Given this approach, we can implement time series modeling approaches such as recurrent neural networks (RNNs) or transformer-based architectures such as large-language-models (LLMs) to capture the time evolution of the system. There is thus a good correspondence between next state prediction in RNNs or next token prediction in LLMs and the ability of emulators and simulators to predict the next neural state [CITE RNN papers on modeling time series; LFADS for example...]. This analogy also works in the case of recent successes of LLMs which are trained on human language behavior (e.g. written text) without a specific model of language generation. LLMs appear to be increasingly able to predict accurate or "viable" outputs in large part because of the flexibility of human language [cite] and the lack of next "ideal" sentence or paragraph.  Thus emulators that implement learned $Q$s may similarly output behavior for next time point. 

%\subsection{Scale-independent emulators can process arbitrary stimuli}

%Assuming that a sufficiently accurate $Q$ can be learned: how would we interact with models implementing $Q$? In particular, while emulators can capture the evolution of neural dynamics at any scale it is not completely obvious how we could provide input into such models given that they do not necessarily model the peripheral nervous system in absolute detail. I.e. how do we "emulate" sensory system transformation of physical information if we don't have a theory or mechanism for doing so? This may appear as one the drawbacks of emulators compared to mechanistic neuroscience. In particular, we have much more complete theories of peripheral nervous system function, for example, such as detailed explanation of how light (i.e. photons) are converted into spiking neurons \cite{doly1994transduction} or how long-term-potentiation works in neural circuits of simpler organisms (e.g. \cite{Kandel1965}). 

%The challenge with emulators is thus how to represent (i.e. input) novel stimuli for which we have no previous training data. For example, a color hue not present in the training data may be challenging to operationalize as input into an emulator model that has not previously "observed" such stimulus.  In mechanistic models, we can assume that the retina - as an interface to the external world - can operationalize any photon wavelength by changing the number and type of photo-receptors activated. More precisely, color experience is achieved by a color mixing steps at various levels of the visual systems but starts with photons of different wavelengths being absorbed by L, M and S cones that have narrow absorption profiles between cone types (yet some variance within cone type). We can conceptualize how we might achieve novel color representation within a mechanistic model of the visual system by simply varying which cones are activated and their proportion based on some hypothesis about the relationship of the novel color to previous colors that we know how to represent (and hope that downstream processes achieve color mixing that we anticipate). 

%We also envision a similar (but perhaps less mechanistic) description of how to emulators could represent and process novel information.\footnote{We envision the possibility of hybrid models where specific mechanistic models of nervous systems such as peripheral sensory processing (which is much better understood) - are coupled with emulators of more complex internal CNS systems.} Thus, emulators would require a transformation of novel stimuli likely via a similar stimulus decomposition or representation where the next-nearest \textit{training-dataset stimulus} is identified as opposed to the next-nearest \textit{color activation} in the above example. 

%First, to repeat, ET does not provide a direct recipe for phenomenal experience, it just states that it is a property of physical systems and it can be emulated at sufficient low scale.

%\subsection{Consciousness}

%ET is essentially a quasi theory of consciousness - it states that bio-physical systems that are \textit{defined}\footnote{WE Can fill out more here.... by whom etc} as being conscious or being conscious can be copied wholesale to other forms or configurations. 


%From Fazekas' paper: Perceptual consciousness and cognitiveaccess: an introduction Peter Fazeka"

%For instance, while ‘global workspace’ [7], ‘higher order thought’ [8] or ‘intermediate level representation’ [9] accountsbuild different varieties of cognitive access or accessibility into the definition of consciousness, ‘local recurrence’ [10] theory denies that such global processing or global avail-ability would be a constitutive part of being conscious.

%\subsection{Odd implications}
%- is it then possible to remove many low-level neural components and just have pure consciousness!?
%- don't answer any weird stuff here..

%An interesting implication is that these types of tests for emulation should drive the definition and the boundary
%- if something other, then the tests DRIVE the definition of EMULATION

%\subsection{Architecture-independence of self-organising systems}
%- While agency or "prediction" may be ultimate principle (?) of self organizing systems, the informational (?) structure of such systems is not prescribed. Can take shape to fit task - and critically accommodate historical/anthropic considerations. 

%See the 4 axioms from the intro(iii) that it individual-specific emulators not generic models that are more likely to emulate all capacities of an organism

%EXPLANTORY POWER (not sure how much though...) ,m

%\subsection{Idiosyncratic evolution: the unnecessary-ness of brain modules}
%- a large elephant in the room is that brain modules and fuctnion likely evolved idiosyncratically.  We certainly konw that despite extreme varaince across brains in tings like single-neuron morphology, there are clear and well defined brain-modules that are generally tasked with specific goals or targets
%- yet, we don't know why the specific structures are precisely the way they are (though many in evo-neuro have interesting plausibility eplxnations; cite; ask Paola). Why is pre-frontal spatially located where it is? But more to the point why does it worry about certain types of balancing between short/long term goals?  Why didn't another part worry about this? Why worry at all - is it necessary because of ecosystems in which brain survive?
%- the answer that we suggest is that almost all of this was driven by random chance in evolution: more specifically, chance occurrences in the development of organisms; 
%- more to the point - 
%- even more computationally - the need for all this compartmentalization may be driven by random idionsyncratic events and efficiency pressures etc; that is, the world may be represntalbe by diffuse completely distributed capacity networks.
%- But the point - really - is that the capacities of brains are driven by both necessary things in the world - but also random things - and things don't have to be the way they are
%- ... not super clear here; I think want to say that the human expeirence is not OBJECTIVE rep of the world; and that there are other ways of experiencing possible.. !? maybe...

%WOULD BE GREAT TO HAVE AN EVO BIO's input here!??!


%\subsection{aren't brains and consciousness RNNs?}
%- e.g. recursion? et unravel rnns and explain how actually their causal componets can be emulated
%- and that there's no magic to sequences of patterns

%- what about low to high level etc

%- what about 


%\subsection{What it's like to be an LLM}
%- be careful, stay mostly away from consciousness material
%- say we don't know, and maybe never will...

%- just point out that the tests for consciousness should be passed by a sufficiently granular emulator 

%- our best guide for now is that physical emulators will increasingly approach biological systems
%- software emulators .. not so clear !?we can then seek to understand internal states by relying - THIS IS OFF THE MARK HERE? 


Our proposal has some limitations. In particular, ET does not describe the content of conscious states or the necessary and sufficient conditions for generating them. ET primarily states that such states can be achieved via artificial activations - or ultimately within completely artificial systems that model biological neural networks in sufficient detail. Additionally, ET proposes that experimentally viable emulators are possible but it remains to be determined whether non-mechanistic, predictive models of neural activity based on neural dynamics can be generated from practical - i.e. non-infinite datasets. 

One additional topic that we did not discuss was the role of physical substrates required for creating synthetic or artificial organisms, such as emulators, which can generate accurate behaviors and may experience phenomenal states.  In our view, there is no physical or conceptual reason for why only so-called "carbon-based" organisms can be good at survival and experience conciousness. This issue is related, among other topics, to the physics of causality and we discuss it in Appendix \ref{sec:physical_substrates}.



%ET is not a theory of consciousness. That is, it does not provide necessary conditions nor the complete sufficient conditions for conscious states. ET states only that at some specifically sufficient emulation scale conscious states will be achieved... In fact, ET suggests that this question may not be completely scientifically answerable [explain why] - and we may have to balance experimental testing with subjectively agreed upon thresholds at which we consider a system to have achieved internal states. 


==> sections/mind_uploading.tex <==
A central theme in artificial intelligence that is linked to understanding brain function is whether we can copy, emulate, or upload brains or minds to digital systems. In this field there increase discussions around humans minds being copied to machines \cite{Chalmers2010-CHATSA} or "mind-uploading" \cite{GOERTZEL2007, Goertzel2012}. Even setting aside the limited scientific progress on this front - there are  significant and unresolved conceptual challenges \cite{Makin2019} including lack of frameworks \cite{Bamford2012-BAMAFF}, the lack of clarity around whether digital copies will experience consciousness or have a personal identity \cite{Haggstrom2017, Pigliucci2014}. In parallel,while we still don't know the necessary or sufficient conditions for conscious states in biological organisms, there are suggestions of a scattershot approach [buttlin] to increase the probability of this. 

==> sections/physical_substrates.tex <==
Here we briefly touch on the question of physical substrates required for behavior and phenomenal states. In particular, in our view, the question of whether only "biological", or "living" or "carbon-based" systems can generate behaviors or experience conscious states is fundamentally a question of causality - not of fundamental physics. For example, there is nothing in the neurobiology that identifies specific building blocks of physical matter (e.g. cellular structure) as necessary conditions for organism-level behaviors (or conscious states). Rather, biology can only identify specific types of processes (i.e. protein interaction) occurring in some substrate (e.g. proteins) as required to cause downstream effects without guaranteeing the necessity of specifically physical composition of such processes. 

ET, as a causality-centered framework, has the flexibility to capture the substrate-independent causality required for generating behaviors and conscious states. For example, if biologists identify that certain specific proteins are necessary for causing a downstream effect, ET can accommodate this by proposing that models that can emulate such downstream effect will capture the causal force of such protein interactions. 

